A drift kinetic model for the expander region of a magnetic mirror

We present a drift kinetic model for the free expansion of a thermal plasma out of a magnetic nozzle. This problem relates to plasma space propulsion systems, natural environments such as the solar wind, and end losses from the expander region of mirror magnetically confined fusion concepts such as the Gas Dynamic Trap. The model incorporates trapped and passing orbit types encountered in the mirror expander geometry and maps to an upstream thermal distribution. This boundary condition and quasineutrality require the generation of an ambipolar potential drop of $\sim5 T_e/e$, forming a thermal barrier for the electrons. The model for the electron and ion velocity distributions and fluid moments is confirmed with data from a fully kinetic simulation. Finally, the model is extended to account for a population of fast sloshing ions arising from neutral beam heating within a magnetic mirror, again resulting in good agreement with a corresponding kinetic simulation.

==> extrarefs.tex <==
@article{skovorodin:2019,
  title={Suppression of secondary emission of electrons from end plate in expander of open trap},
  author={Skovorodin, DI},
  journal={Physics of Plasmas},
  volume={26},
  number={1},
  pages={012503},
  year={2019},
  publisher={AIP Publishing LLC}
}




@article{soldatkina:2017,
  title={Influence of the magnetic field expansion on the core plasma in an axisymmetric mirror trap},
  author={Soldatkina, E and Anikeev, M and Bagryansky, P and Korzhavina, M and Maximov, V and Savkin, V and Yakovlev, D and Yushmanov, P and Dunaevsky, A},
  journal={Physics of Plasmas},
  volume={24},
  number={2},
  pages={022505},
  year={2017},
  publisher={AIP Publishing LLC}
}



@article{kotelnikov1985,
  title={Effects of ambipolar potential in a two-component gasdynamic confinement system},
  author={Kotel'nikov, IA and Ryutov, DD},
  journal={Soviet Journal of Plasma Physics},
  volume={11},
  number={10},
  pages={655--660},
  year={1985}
}

@article{ryutov2005,
  title={Axial electron heat loss from mirror devices revisited},
  author={Ryutov, DD},
  journal={Fusion science and technology},
  volume={47},
  number={1T},
  pages={148--154},
  year={2005},
  publisher={Taylor \& Francis}
}

@article{maximov2004,
  title={Spatial profiles of fusion product flux in the gas dynamic trap with deuterium neutral beam injection},
  author={Maximov, VV and Anikeev, AV and Bagryansky, PA and Ivanov, AA and Lizunov, AA and Murakhtin, SV and Noack, K and Prikhodko, VV},
  journal={Nuclear Fusion},
  volume={44},
  number={4},
  pages={542},
  year={2004},
  publisher={IOP Publishing}
}

@article{coensgen1975,
  title={Stabilization of a Neutral-Beam—Sustained, Mirror-Confined Plasma},
  author={Coensgen, FH and Cummins, WF and Logan, BG and Molvik, AW and Nexsen, WE and Simonen, TC and Stallard, BW and Turner, WC},
  journal={Physical Review Letters},
  volume={35},
  number={22},
  pages={1501},
  year={1975},
  publisher={APS}
}


@article{yushmanov1966,
  title={Confinement of Slow Ions of a Plasma with Positive Potential in a Mirror Trap},
  author={Yushmanov, EE},
  journal={SOVIET PHYSICS JETP},
  volume={22},
  number={2},
  year={1966}
}

@article{ivanov2017,
  title={Gas dynamic trap: experimental results and future prospects},
  author={Ivanov, Alexander Alexandrovich and Prikhodko, Vadim Vadimovich},
  journal={Physics-Uspekhi},
  volume={60},
  number={5},
  pages={509},
  year={2017},
  publisher={IOP Publishing}
}
